A Study on Learning and Simulating Personalized Car-Following Driving Style

Automated vehicles are gradually entering people's daily life to provide a comfortable driving experience for the users. The generic and user-agnostic automated vehicles have limited ability to accommodate the different driving styles of different users. This limitation not only impacts users' satisfaction but also causes safety concerns. Learning from user demonstrations can provide direct insights regarding users' driving preferences. However, it is difficult to understand a driver's preference with limited data. In this study, we use a model-free inverse reinforcement learning method to study drivers' characteristics in the car-following scenario from a naturalistic driving dataset, and show this method is capable of representing users' preferences with reward functions. In order to predict the driving styles for drivers with limited data, we apply Gaussian Mixture Models and compute the similarity of a specific driver to the clusters of drivers. We design a personalized adaptive cruise control (P-ACC) system through a partially observable Markov decision process (POMDP) model. The reward function with the model to mimic drivers' driving style is integrated, with a constraint on the relative distance to ensure driving safety. Prediction of the driving styles achieves 85.7% accuracy with the data of less than 10 car-following events. The model-based experimental driving trajectories demonstrate that the P-ACC system can provide a personalized driving experience.

==> tables/table_POMDP_Definition.tex <==
%%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t] \centering 
\caption{Definition of the trust-POMDP model} 
\label{tableDefinition} 
\begin{tabular}{l|llp{8cm}}
\hline
                       & Meaning           & Values                  & Explanation         \\ \hline\hline
\multirow{2}{*}{State} & World state $x$     & $x_{A},x_{end}, x_{BT},x_{BP},...x_{KT},x_{KP}$ & $x_{A}$ indicates the start point,$x_{BT}$ indicates human has taken over on the way to Position A, $x_{BP}$ indicates human has stayed put.      \\ \cline{2-4} 
                       & Trust state $T$ & $1,...,7$           &The trust that human holds on the autonomous driving system.   \\ \hline
Action                 & Vehicle direction $a$  & $a_{left},a_{straight},a_{right}$             & The direction that the autonomous driving system selects to drive.     \\ \hline
Observation            & Human behavior $o$    & take-over, stay-put     & Human's decision on how to maneuver the incident.\\
\bottomrule
\end{tabular}
\end{table*}
%%

==> tables/table_reward_function.tex <==
\begin{table}[t]\centering
\caption{Reward function} 
\label{tableReward} 
\begin{tabular}{l|ccccc}

\hline
          & Truck & Obstacle & Pedestrian & Empty Road \\ \hline\hline
Stay-put  & 1     & 2        & 3          & 5          \\
Take-over & 0     & 0        & 0          & 0          \\
Failure  & 0    & -6       & -9         & 0          \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/table_trust_questionnaire.tex <==
\begin{table}[t]\centering
\caption{Muir's questionnaire} 
\label{tabletrustQuestionnaire}
\begin{tabular}{p{8cm}}
\hline
Q1. After watching the video on the left, how likely do you think the autopilot can safely maneuver this incident? \\
Q2. Based on your current trust in the autopilot, do you wish to take over and drive manually or are you comfortable with autonomous driving if you were in the situation displayed in the video?                                                    \\
Q3. Based on your experience so far, how would you update your trust in the  autopilot?                         \\
Q4. To what extent can you count on the autopilot to do its job?                  \\
 \hline
\end{tabular}
\end{table}
